Low-Rank plus Sparse Decomposition of Covariance Matrices using Neural Network Parametrization

This paper revisits the problem of decomposing a positive semidefinite matrix as a sum of a matrix with a given rank plus a sparse matrix. An immediate application can be found in portfolio optimization, when the matrix to be decomposed is the covariance between the different assets in the portfolio. Our approach consists in representing the low-rank part of the solution as the product $MM^{T}$, where $M$ is a rectangular matrix of appropriate size, parametrized by the coefficients of a deep neural network. We then use a gradient descent algorithm to minimize an appropriate loss function over the parameters of the network. We deduce its convergence rate to a local optimum from the Lipschitz smoothness of our loss function. We show that the rate of convergence grows polynomially in the dimensions of the input, output, and the size of each of the hidden layers.

==> images/simulated/batch/table.tex <==
\begin{center}
\resizebox{ \textwidth}{!}{
\begin{tabular}{*{4}{c}*{6}{c}}\\
\hline
N & $r(L_0)$ & f & $s(S_0)$  &Algo & $r(L)$  & $s(S)$ & rel.error(S)& rel.error(L)\\
  \hline\hline
 10 & 2 & 2 & 0.95 &FPCP & 2.0 (0.0) & 0.75 (0.14) & 2.08 (1.23) & 1.29 (0.28) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 2.0 (0.0) &\cellcolor{lightgray} 0.02 (0.02) &\cellcolor{lightgray} 3.36 (1.74) &\cellcolor{lightgray} 0.42 (0.16) \\ 
\hline
\end{tabular}}
\end{center} 10 & 2 & 2 & 0.95 &FPCP & 2.0 (0.0) & 0.74 (0.12) & 1.81 (1.31) & 0.29 (0.12) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 2.0 (0.0) &\cellcolor{lightgray} 0.02 (0.02) &\cellcolor{lightgray} 3.36 (1.74) &\cellcolor{lightgray} 0.42 (0.16) \\ 
\hline
\end{tabular}}
\end{center} 10 & 2 & 2 & 0.95 &FPCP & 2.0 (0.0) & 0.76 (0.14) & 1.65 (1.21) & 0.27 (0.13) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 2.0 (0.0) &\cellcolor{lightgray} 0.02 (0.02) &\cellcolor{lightgray} 3.31 (1.85) &\cellcolor{lightgray} 0.41 (0.16) \\ 
\hline
\end{tabular}}
\end{center} 10 & 2 & 2 & 0.95 &FPCP & 2.0 (0.0) & 0.55 (0.0) & 2.19 (0.0) & 0.27 (0.0) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 2.0 (0.0) &\cellcolor{lightgray} 0.0 (0.0) &\cellcolor{lightgray} 4.52 (0.0) &\cellcolor{lightgray} 0.41 (0.0) \\ 
\hline
\end{tabular}}
\end{center} 10 & 2 & 2 & 0.95 &FPCP & 2.0 (0.0) & 0.77 (0.17) & 1.67 (1.42) & 0.28 (0.13) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 2.0 (0.0) &\cellcolor{lightgray} 0.01 (0.02) &\cellcolor{lightgray} 3.6 (1.98) &\cellcolor{lightgray} 0.48 (0.19) \\ 
\hline
\end{tabular}}
\end{center} 10 & 2 & 2 & 0.95 &FPCP & 2.0 (0.0) & 0.77 (0.17) & 1.67 (1.42) & 0.28 (0.13) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 2.0 (0.0) &\cellcolor{lightgray} 0.01 (0.02) &\cellcolor{lightgray} 3.6 (1.98) &\cellcolor{lightgray} 0.48 (0.19) \\ 
\hline
\end{tabular}}
\end{center} 10 & 2 & 2 & 0.95 &FPCP & 2.0 (0.0) & 0.74 (0.19) & 1.83 (1.1) & 0.33 (0.06) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 2.0 (0.0) &\cellcolor{lightgray} 0.04 (0.03) &\cellcolor{lightgray} 2.75 (1.77) &\cellcolor{lightgray} 0.39 (0.21) \\ 
\hline
\end{tabular}}
\end{center} 10 & 2 & 2 & 0.95 &FPCP & 2.0 (0.0) & 0.74 (0.19) & 1.83 (1.1) & 0.33 (0.06) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 2.0 (0.0) &\cellcolor{lightgray} 0.04 (0.03) &\cellcolor{lightgray} 2.75 (1.77) &\cellcolor{lightgray} 0.39 (0.21) \\ 
\hline
\end{tabular}}
\end{center} 10 & 2 & 2 & 0.95 &FPCP & 2.0 (0.0) & 0.74 (0.19) & 1.83 (1.1) & 0.33 (0.06) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 2.0 (0.0) &\cellcolor{lightgray} 0.04 (0.03) &\cellcolor{lightgray} 2.75 (1.77) &\cellcolor{lightgray} 0.39 (0.21) \\ 
\hline
\end{tabular}}
\end{center} 10 & 2 & 2 & 0.95 &FPCP & 2.0 (0.0) & 0.74 (0.19) & 1.83 (1.1) & 0.33 (0.06) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 2.0 (0.0) &\cellcolor{lightgray} 0.04 (0.03) &\cellcolor{lightgray} 2.75 (1.77) &\cellcolor{lightgray} 0.39 (0.21) \\ 
\hline
\end{tabular}}
\end{center} 10 & 2 & 2 & 0.95 &FPCP & 2.0 (0.0) & 0.74 (0.19) & 1.83 (1.1) & 0.33 (0.06) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 2.0 (0.0) &\cellcolor{lightgray} 0.04 (0.03) &\cellcolor{lightgray} 2.75 (1.77) &\cellcolor{lightgray} 0.39 (0.21) \\ 
\hline
\end{tabular}}
\end{center} 10 & 2 & 2 & 0.95 &FPCP & 2.0 (0.0) & 0.74 (0.19) & 1.83 (1.1) & 0.33 (0.06) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 2.0 (0.0) &\cellcolor{lightgray} 0.04 (0.03) &\cellcolor{lightgray} 2.75 (1.77) &\cellcolor{lightgray} 0.39 (0.21) \\ 
\hline
\end{tabular}}
\end{center} 10 & 2 & 2 & 0.95 &FPCP & 2.0 (0.0) & 0.74 (0.19) & 1.83 (1.1) & 0.33 (0.06) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 2.0 (0.0) &\cellcolor{lightgray} 0.04 (0.03) &\cellcolor{lightgray} 2.75 (1.77) &\cellcolor{lightgray} 0.39 (0.21) \\ 
\hline
\end{tabular}}
\end{center} 10 & 2 & 2 & 0.95 &FPCP & 2.0 (0.0) & 0.74 (0.19) & 1.83 (1.1) & 0.33 (0.06) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 2.0 (0.0) &\cellcolor{lightgray} 0.04 (0.03) &\cellcolor{lightgray} 2.75 (1.77) &\cellcolor{lightgray} 0.39 (0.21) \\ 
\hline
\end{tabular}}
\end{center} 10 & 2 & 2 & 0.95 &FPCP & 2.0 (0.0) & 0.74 (0.19) & 1.83 (1.1) & 0.33 (0.06) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 2.0 (0.0) &\cellcolor{lightgray} 0.04 (0.03) &\cellcolor{lightgray} 2.75 (1.77) &\cellcolor{lightgray} 0.39 (0.21) \\ 
\hline
\end{tabular}}
\end{center} 10 & 2 & 2 & 0.95 &FPCP & 2.0 (0.0) & 0.74 (0.19) & 1.83 (1.1) & 0.33 (0.06) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 2.0 (0.0) &\cellcolor{lightgray} 0.04 (0.03) &\cellcolor{lightgray} 2.75 (1.77) &\cellcolor{lightgray} 0.39 (0.21) \\ 
\hline
\end{tabular}}
\end{center} 10 & 2 & 2 & 0.95 &FPCP & 2.0 (0.0) & 0.74 (0.19) & 1.83 (1.1) & 0.33 (0.06) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 2.0 (0.0) &\cellcolor{lightgray} 0.04 (0.03) &\cellcolor{lightgray} 2.75 (1.77) &\cellcolor{lightgray} 0.39 (0.21) \\ 
\hline
\end{tabular}}
\end{center} 10 & 2 & 2 & 0.95 &FPCP & 2.0 (0.0) & 0.74 (0.19) & 1.83 (1.1) & 0.33 (0.06) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 2.0 (0.0) &\cellcolor{lightgray} 0.04 (0.03) &\cellcolor{lightgray} 2.75 (1.77) &\cellcolor{lightgray} 0.39 (0.21) \\ 
\hline
\end{tabular}}
\end{center} 10 & 2 & 2 & 0.95 &FPCP & 2.0 (0.0) & 0.74 (0.19) & 1.83 (1.1) & 0.33 (0.06) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 2.0 (0.0) &\cellcolor{lightgray} 0.04 (0.03) &\cellcolor{lightgray} 2.75 (1.77) &\cellcolor{lightgray} 0.39 (0.21) \\ 
\hline
\end{tabular}}
\end{center} 10 & 2 & 2 & 0.95 &FPCP & 2.0 (0.0) & 0.74 (0.19) & 1.83 (1.1) & 0.33 (0.06) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 2.0 (0.0) &\cellcolor{lightgray} 0.04 (0.03) &\cellcolor{lightgray} 2.75 (1.77) &\cellcolor{lightgray} 0.39 (0.21) \\ 
\hline
\end{tabular}}
\end{center} 10 & 2 & 2 & 0.95 &FPCP & 2.0 (0.0) & 0.74 (0.19) & 1.83 (1.1) & 0.33 (0.06) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 2.0 (0.0) &\cellcolor{lightgray} 0.04 (0.03) &\cellcolor{lightgray} 2.75 (1.77) &\cellcolor{lightgray} 0.39 (0.21) \\ 
\hline
\end{tabular}}
\end{center} 10 & 2 & 2 & 0.95 &FPCP & 2.0 (0.0) & 0.74 (0.19) & 1.83 (1.1) & 0.33 (0.06) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 2.0 (0.0) &\cellcolor{lightgray} 0.04 (0.03) &\cellcolor{lightgray} 2.75 (1.77) &\cellcolor{lightgray} 0.39 (0.21) \\ 
\hline
\end{tabular}}
\end{center}

==> images/simulated/table.tex <==
\begin{center}
\label{table}
\resizebox{12cm}{!}{
\begin{tabular}{*{4}{c}*{6}{c}}\\
\hline
n & $r(L_0)$ & k & $s(S_0)$  &Algo & $r(L)$  & $s(S)$ & rel.error(S)& rel.error(L)\\
  \hline\hline
 100 & 5 & 5 & 0.6 &FPCP & 5.0 (0.0) & 0.08 (0.0) & 0.36 (0.03) & 0.78 (0.03) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 5.0 (0.0) &\cellcolor{lightgray} 0.1 (0.03) &\cellcolor{lightgray} 0.01 (0.01) &\cellcolor{lightgray} 0.03 (0.01) \\ 
 100 & 5 & 5 & 0.95 &FPCP & 5.0 (0.0) & 0.1 (0.01) & 3.87 (0.38) & 0.72 (0.02) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 5.0 (0.0) &\cellcolor{lightgray} 0.25 (0.04) &\cellcolor{lightgray} 0.08 (0.02) &\cellcolor{lightgray} 0.01 (0.0) \\ 
 100 & 5 & 10 & 0.6 &FPCP & 7.2 (0.4) & 0.15 (0.01) & 0.3 (0.03) & 0.64 (0.04) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 10.0 (0.0) &\cellcolor{lightgray} 0.11 (0.02) &\cellcolor{lightgray} 0.03 (0.0) &\cellcolor{lightgray} 0.06 (0.01) \\ 
 100 & 5 & 10 & 0.95 &FPCP & 7.5 (0.5) & 0.22 (0.02) & 3.06 (0.35) & 0.58 (0.02) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 10.0 (0.0) &\cellcolor{lightgray} 0.25 (0.07) &\cellcolor{lightgray} 0.18 (0.06) &\cellcolor{lightgray} 0.03 (0.01) \\ 
 100 & 5 & 20 & 0.6 &FPCP & 9.7 (0.46) & 0.31 (0.02) & 0.19 (0.02) & 0.41 (0.04) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 20.0 (0.0) &\cellcolor{lightgray} 0.08 (0.02) &\cellcolor{lightgray} 0.05 (0.01) &\cellcolor{lightgray} 0.1 (0.01) \\ 
 100 & 5 & 20 & 0.95 &FPCP & 10.1 (0.3) & 0.59 (0.05) & 1.8 (0.3) & 0.34 (0.03) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 20.0 (0.0) &\cellcolor{lightgray} 0.22 (0.05) &\cellcolor{lightgray} 0.32 (0.11) &\cellcolor{lightgray} 0.06 (0.02) \\ 
&&&&&&&&& \\ 
 100 & 10 & 5 & 0.6 &FPCP & 5.0 (0.0) & 0.04 (0.0) & 0.57 (0.03) & 0.86 (0.01) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 5.0 (0.0) &\cellcolor{lightgray} 0.01 (0.0) &\cellcolor{lightgray} 0.36 (0.02) &\cellcolor{lightgray} 0.53 (0.02) \\ 
 100 & 10 & 5 & 0.95 &FPCP & 5.0 (0.0) & 0.04 (0.0) & 6.56 (0.21) & 0.84 (0.01) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 5.0 (0.0) &\cellcolor{lightgray} 0.01 (0.0) &\cellcolor{lightgray} 4.35 (0.18) &\cellcolor{lightgray} 0.54 (0.02) \\ 
 100 & 10 & 10 & 0.6 &FPCP & 8.2 (0.4) & 0.06 (0.01) & 0.51 (0.03) & 0.77 (0.01) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 10.0 (0.0) &\cellcolor{lightgray} 0.06 (0.02) &\cellcolor{lightgray} 0.03 (0.01) &\cellcolor{lightgray} 0.04 (0.01) \\ 
 100 & 10 & 10 & 0.95 &FPCP & 9.0 (0.0) & 0.07 (0.01) & 5.78 (0.2) & 0.74 (0.01) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 10.0 (0.0) &\cellcolor{lightgray} 0.16 (0.05) &\cellcolor{lightgray} 0.14 (0.05) &\cellcolor{lightgray} 0.02 (0.01) \\ 
 100 & 10 & 20 & 0.6 &FPCP & 11.5 (0.5) & 0.14 (0.01) & 0.38 (0.03) & 0.57 (0.01) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 20.0 (0.0) &\cellcolor{lightgray} 0.06 (0.01) &\cellcolor{lightgray} 0.05 (0.01) &\cellcolor{lightgray} 0.08 (0.01) \\ 
 100 & 10 & 20 & 0.95 &FPCP & 12.0 (0.0) & 0.19 (0.01) & 4.09 (0.2) & 0.53 (0.01) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 20.0 (0.0) &\cellcolor{lightgray} 0.17 (0.04) &\cellcolor{lightgray} 0.32 (0.08) &\cellcolor{lightgray} 0.04 (0.01) \\ 
&&&&&&&&& \\ 
 100 & 20 & 5 & 0.6 &FPCP & 4.6 (0.49) & 0.03 (0.0) & 0.92 (0.03) & 0.9 (0.01) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 5.0 (0.0) &\cellcolor{lightgray} 0.01 (0.0) &\cellcolor{lightgray} 0.71 (0.03) &\cellcolor{lightgray} 0.69 (0.02) \\ 
 100 & 20 & 5 & 0.95 &FPCP & 5.0 (0.0) & 0.03 (0.0) & 10.49 (0.51) & 0.9 (0.01) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 5.0 (0.0) &\cellcolor{lightgray} 0.01 (0.0) &\cellcolor{lightgray} 8.21 (0.38) &\cellcolor{lightgray} 0.69 (0.02) \\ 
 100 & 20 & 10 & 0.6 &FPCP & 7.3 (0.46) & 0.03 (0.0) & 0.87 (0.03) & 0.86 (0.01) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 10.0 (0.0) &\cellcolor{lightgray} 0.01 (0.0) &\cellcolor{lightgray} 0.46 (0.02) &\cellcolor{lightgray} 0.45 (0.02) \\ 
 100 & 20 & 10 & 0.95 &FPCP & 8.1 (0.3) & 0.04 (0.0) & 9.96 (0.48) & 0.85 (0.01) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 10.0 (0.0) &\cellcolor{lightgray} 0.01 (0.0) &\cellcolor{lightgray} 5.44 (0.25) &\cellcolor{lightgray} 0.46 (0.02) \\ 
 100 & 20 & 20 & 0.6 &FPCP & 11.4 (0.49) & 0.06 (0.01) & 0.77 (0.03) & 0.76 (0.01) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 20.0 (0.0) &\cellcolor{lightgray} 0.04 (0.0) &\cellcolor{lightgray} 0.04 (0.01) &\cellcolor{lightgray} 0.04 (0.0) \\ 
 100 & 20 & 20 & 0.95 &FPCP & 12.1 (0.3) & 0.07 (0.0) & 8.66 (0.42) & 0.74 (0.01) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 20.0 (0.0) &\cellcolor{lightgray} 0.11 (0.02) &\cellcolor{lightgray} 0.21 (0.08) &\cellcolor{lightgray} 0.02 (0.01) \\ 
\\
 200 & 5 & 5 & 0.95 &FPCP & 5.0 (0.0) & 0.06 (0.0) & 2.84 (0.15) & 0.78 (0.01) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 5.0 (0.0) &\cellcolor{lightgray} 0.18 (0.02) &\cellcolor{lightgray} 0.08 (0.01) &\cellcolor{lightgray} 0.02 (0.0) \\ 
 400 & 10 & 10 & 0.95 &FPCP & 7.4 (0.49) & 0.02 (0.0) & 3.1 (0.07) & 0.86 (0.0) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 10.0 (0.0) &\cellcolor{lightgray} 0.12 (0.05) &\cellcolor{lightgray} 0.08 (0.03) &\cellcolor{lightgray} 0.02 (0.01) \\ 
 800 & 20 & 20 & 0.95 &FPCP & 9.0 (0.0) & 0.01 (0.0) & 3.29 (0.04) & 0.92 (0.0) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 18.1 (5.7) &\cellcolor{lightgray} 0.04 (0.02) &\cellcolor{lightgray} 1.16 (1.59) &\cellcolor{lightgray} 0.32 (0.44) \\ 
 1600 & 40 & 40 & 0.95 &FPCP & 10.0 (0.0) & 0.01 (0.0) & 3.42 (0.02) & 0.96 (0.0) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 16.6 (19.11) &\cellcolor{lightgray} 0.01 (0.01) &\cellcolor{lightgray} 2.26 (1.63) &\cellcolor{lightgray} 0.63 (0.45) \\ 
\hline
\end{tabular}}
\end{center}

==> images/simulated/table_high.tex <==
\begin{center}
\resizebox{12cm}{!}{
\begin{tabular}{*{4}{c}*{6}{c}}\\
\hline
N & $r(L_0)$ & f & $s(S_0)$  &Algo & $r(L)$  & $s(S)$ & rel.error(S)& rel.error(L)\\
  \hline\hline
 200 & 5 & 5 & 0.95 &FPCP & 5.0 (0.0) & 0.06 (0.0) & 2.84 (0.15) & 0.78 (0.01) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 5.0 (0.0) &\cellcolor{lightgray} 0.18 (0.02) &\cellcolor{lightgray} 0.08 (0.01) &\cellcolor{lightgray} 0.02 (0.0) \\ 
 400 & 10 & 10 & 0.95 &FPCP & 7.4 (0.49) & 0.02 (0.0) & 3.1 (0.07) & 0.86 (0.0) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 10.0 (0.0) &\cellcolor{lightgray} 0.12 (0.05) &\cellcolor{lightgray} 0.08 (0.03) &\cellcolor{lightgray} 0.02 (0.01) \\ 
 800 & 20 & 20 & 0.95 &FPCP & 9.0 (0.0) & 0.01 (0.0) & 3.29 (0.04) & 0.92 (0.0) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 18.1 (5.7) &\cellcolor{lightgray} 0.04 (0.02) &\cellcolor{lightgray} 1.16 (1.59) &\cellcolor{lightgray} 0.32 (0.44) \\ 
 1600 & 40 & 40 & 0.95 &FPCP & 10.0 (0.0) & 0.01 (0.0) & 3.42 (0.02) & 0.96 (0.0) \\ 
&&&&\cellcolor{lightgray} DNN &\cellcolor{lightgray} 16.6 (19.11) &\cellcolor{lightgray} 0.01 (0.01) &\cellcolor{lightgray} 2.26 (1.63) &\cellcolor{lightgray} 0.63 (0.45) \\ 
\hline
\end{tabular}}
\end{center}
